CITlab ARGUS for historical handwritten documents

We describe CITlab's recognition system for the HTRtS competition attached to the 14. International Conference on Frontiers in Handwriting Recognition, ICFHR 2014. The task comprises the recognition of historical handwritten documents. The core algorithms of our system are based on multi-dimensional recurrent neural networks (MDRNN) and connectionist temporal classification (CTC). The software modules behind that as well as the basic utility technologies are essentially powered by PLANET's ARGUS framework for intelligent text recognition and image processing.

==> tableArch.tex <==
\begin{table}[h]
  \centering
  \begin{tabular}[t]{c@{\hspace{3em}}*{3}{c}}
    & \multicolumn{3}{c}{number of} \\ \cline{2-4} \\[-.75em]
    network & cells & trainable weights & output neurons \\ \hline \\[-.75em]
    $\mathcal{N}_1$ & 1900 & 958387 & 56 \\
    $\mathcal{N}_2$ & 1166 & 363477 & 56 \\
    $\mathcal{N}_3$ & 1166 & 363477 & 56 \\
    $\mathcal{R}_1$ & 1900 & 1006387 & 56 \\
    $\mathcal{R}_2$ & 1900 & 1006387 & 56 \\
    $\mathcal{A}$ & 1869 & 933556 & 25 \\
    $\mathcal{M}$ & 1851 & 967138 & 7 \\
    $\mathcal{B}_1$ & 1899 & 1005586 & 55 \\
    $\mathcal{B}_2$ & 1532 & 655747 & 55 \\
  \end{tabular}
  \caption{Architecture parameters}
  \label{tab:tableArch}
\end{table}

